Multi-scale closed-loop melt pool control for LPBF via policy optimization

Laser powder bed fusion (LPBF) is a metal additive manufacturing process where temperature stabilization is of vital importance to avoid defects such as distortion and cracking. Existing control methods require manual tuning, increasing the risk of part failure when printing complex geometries. This paper introduces a dual-loop, data-driven control strategy to stabilize the surface temperature, ensuring robustness and near-optimal performance in the presence of disturbances. The proposed method integrates (i) an in-layer linear output feedback control with gains optimized through policy gradient, and (ii) a layer-to-layer feedforward control combining temperature trajectory optimization and iterative learning control. Simulation results show that the multi-scale controller effectively stabilizes the temperature even under significant model mismatch and measurement noise. Experimental results demonstrate that a simplified, hardware-constrained version of this method matches the state-of-the-art performance of in-situ data-driven methods, reducing mean tracking error by 3.4% and mean input-constraint violation by 47.5% relative to a Bayesian Optimization-tuned baseline. For this physical LPBF validation, the controller is tuned entirely offline using uncontrolled print data from a single calibration layer. Our experiments also demonstrate a new class of high-frequency excitation dynamics that result in reduced vector head swelling, opening up new avenues of research in the additive manufacturing community. This work marks one of the first successful applications of sim-to-real policy optimization in LPBF processes.

==> graphics/colors.tex <==
\definecolor{chocolate2168224}{RGB}{216,82,24}
\definecolor{darkcyan0113188}{RGB}{0,113,188}
\definecolor{purple12546141}{RGB}{125,46,141}

\definecolor{brown1611946}{RGB}{161,19,46}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}

\definecolor{matlabYellow}{RGB}{255, 127, 14}
\definecolor{matlabRed}{RGB}{214, 39, 40}
\colorlet{newBlue}{darkcyan0113188}
\definecolor{newlblue}{RGB}{77,190,238}
\definecolor{newGreen}{RGB}{44,160,44}

% MATLAB default color order
\definecolor{matlabBlue}{RGB}{0,114,189}    % [0, 0.4470, 0.7410]
\definecolor{matlabRed}{RGB}{217,83,25}     % [0.8500, 0.3250, 0.0980]
\definecolor{matlabYellow}{RGB}{237,177,32} % [0.9290, 0.6940, 0.1250]
\definecolor{matlabPurple}{RGB}{126,47,142} % [0.4940, 0.1840, 0.5560]
\definecolor{matlabGreen}{RGB}{119,172,48}  % [0.4660, 0.6740, 0.1880]
\definecolor{matlabCyan}{RGB}{77,190,238}   % [0.3010, 0.7450, 0.9330]
\definecolor{matlabBurgundy}{RGB}{162,20,47}% [0.6350, 0.0780, 0.1840]

% Matplotlib tab: colors (Tableau 10)
\definecolor{tabBlue}{RGB}{31,119,180}      % tab:blue
\definecolor{tabOrange}{RGB}{255,127,14}    % tab:orange
\definecolor{tabGreen}{RGB}{44,160,44}      % tab:green
\definecolor{tabRed}{RGB}{214,39,40}        % tab:red
\definecolor{tabPurple}{RGB}{148,103,189}   % tab:purple
\definecolor{tabBrown}{RGB}{140,86,75}      % tab:brown
\definecolor{tabPink}{RGB}{227,119,194}     % tab:pink
\definecolor{tabGray}{RGB}{127,127,127}     % tab:gray
\definecolor{tabOlive}{RGB}{188,189,34}     % tab:olive
\definecolor{tabCyan}{RGB}{23,190,207}      % tab:cyan


% progression of blue colors
\definecolor{tabBlueLight1}{RGB}{82,153,204}
\definecolor{tabBlueLight2}{RGB}{133,187,224}
\definecolor{tabBlueLight3}{RGB}{184,221,242}

% \pgfplotsset{ every non boxed x axis/.append style={x axis line style=-},
%      every non boxed y axis/.append style={y axis line style=-}}

% \pgfplotsset{line1/.style={
%     very thick,
%     darkcyan0113188,
%     mark=square*, 
%     mark size=0.75, 
%     mark options={solid}
% }}
% \pgfplotsset{line2/.style={
%     very thick,
%     purple12546141,
%     dash pattern=on 5.25pt off 1.75pt on 1.75pt off 1.75pt
% }}
% \pgfplotsset{line3/.style={
%     very thick,
%     chocolate2168224,
%     dash pattern=on 1.75pt off 1.75pt,
%     mark=*,
%     mark size=0.625,
%     mark options={solid}
% }}
\pgfplotsset{blue_solid/.style={
    very thick,
    tabBlue,
    % mark=square*, 
    % mark size=0.75, 
    % mark options={solid}
}}
\pgfplotsset{blue_dashed/.style={
    very thick,
    tabBlue,
    dash pattern=on 5pt off 2pt
    % mark=square*, 
    % mark size=0.75, 
    % mark options={solid}
}}
\pgfplotsset{green_solid/.style={
    very thick,
    tabGreen,
    % mark=square*, 
    % mark size=0.75, 
    % mark options={solid}
}}
\pgfplotsset{blue_dashdot/.style={
    very thick,
    tabBlue,
    dash pattern=on 5.25pt off 1.75pt on 1.75pt off 1.75pt
    % mark=square*, 
    % mark size=0.75, 
    % mark options={solid}
}}
\pgfplotsset{orange_solid/.style={
    very thick,
    tabOrange
    % dash pattern=on 5.25pt off 1.75pt on 1.75pt off 1.75pt
}}
\pgfplotsset{orange_dashdot/.style={
    very thick,
    tabOrange,
    dash pattern=on 5.25pt off 1.75pt on 1.75pt off 1.75pt
}}
\pgfplotsset{orange_dashed/.style={
    very thick,
    tabOrange,
    dash pattern=on 5pt off 2pt
}}
\pgfplotsset{red_dashed/.style={
    very thick,
    tabRed,
    dash pattern=on 5pt off 2pt
    % mark=*,
    % mark size=0.625,
    % mark options={solid}
}}
\pgfplotsset{red_dashdot/.style={
    very thick,
    tabRed,
    dash pattern=on 5.25pt off 1.75pt on 1.75pt off 1.75pt,
    % mark=*,
    % mark size=0.625,
    % mark options={solid}
}}
\pgfplotsset{red_solid/.style={
    very thick,
    tabRed,
    % dash pattern=on 5.25pt off 1.75pt on 1.75pt off 1.75pt,
    % mark=*,
    % mark size=0.625,
    % mark options={solid}
}}
\pgfplotsset{gray_dashed/.style={
    thick,
    darkgray176,
    dash pattern=on 5.25pt off 1.75pt on 1.75pt off 1.75pt,
    % mark=*,
    % mark size=0.625,
    % mark options={solid}
}}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

% \definecolor{brown1611946}{RGB}{161,19,46}
% \definecolor{chocolate2168224}{RGB}{216,82,24}
% \definecolor{darkcyan0113188}{RGB}{0,113,188}
% \definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gray127}{RGB}{127,127,127}

==> graphics/picture_header.tex <==
\usepackage{amsmath,amssymb,amsfonts,amsthm}
\usepackage{pifont}
\usepackage{tabularx}
\usepackage{xcolor}
\usepackage{array}
\usepackage{dsfont}
\usepackage{commath}
\usepackage{placeins}
\let\argmax\relax
\let\argmin\relax
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\R}{\mathbb{R}}
\usepackage{siunitx}
\sisetup{detect-all}

% Fonts
\let\Bbbk\relax
\usepackage[cmintegrals,cmbraces,varbb]{newtxmath} % Math font
\usepackage[cal=cm,bb=ams]{mathalpha} % Improve calligraphic and bb math
\renewcommand{\ttfamily}{\fontencoding{T1}\fontfamily{lmtt}\selectfont}

\let\allfigurefontsize\footnotesize

\definecolor{brown1611946}{RGB}{161,19,46}
\definecolor{chocolate2168224}{RGB}{216,82,24}
\definecolor{darkcyan0113188}{RGB}{0,113,188}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\colorlet{mygreen}{darkorange25512714}
\colorlet{myblue}{darkcyan0113188}

\usepackage{pgfplots}
\DeclareUnicodeCharacter{2212}{−}
\usepgfplotslibrary{groupplots,dateplot}
\usetikzlibrary{patterns,shapes.arrows}
\pgfplotsset{compat=newest}
\usetikzlibrary{decorations.markings}

\usepackage{pgfplotstable}
\usepgfplotslibrary{statistics}

\usepackage{tikz}
\usetikzlibrary{spy}
\usetikzlibrary{calc}
\usetikzlibrary{arrows.meta, positioning, shapes.geometric, backgrounds, fit}
\tikzset{
  block/.style = {rectangle, draw, align=center, minimum height=2em, minimum width=7.5em},
  startstop/.style = {ellipse, draw, minimum height=2em, minimum width=5em, align=center},
  decision/.style = {diamond, draw, aspect=2, inner sep=1pt, align=center},
  line/.style = {draw, -{Latex[width=2mm,length=2mm]}},
  stage/.style = {font=\small\bfseries}
}

==> sections/materials_and_methods/experiment_design.tex <==




\subsection{Experimental Setup and Simulation Parameter Calibration} \label{sec:experiment_design:experimental}

\begin{figure}[b]
\centering
\scalebox{0.9}{
    \import{./graphics/svgs/}{block_real_experiment.pdf_tex}
}
\caption{The simplified control architecture for the physical LPBF.}
\label{fig:SLMSimplifiedControlArchitecture}
\end{figure}

\eb{Due to the limitations with the physical LPBF setup in this study, we performed simplifications to the proposed multi-scale control method in~\cref{sec:methods_control}. \cref{fig:SLMSimplifiedControlArchitecture} summarizes the adaptations on the experimental setup. 
Two key adjustments are: 
\begin{itemize}
    \item The setup is not capable of run-time adjustments of layer-to-layer parameters together with the PI controller, which is a common limitation with existing machines. Therefore, we design the layer-to-layer control input as a fixed feedforward signal for the PI controller.
    \item The input projection for the in-layer controller is not utilized in this study to avoid nonlinearities caused by input saturation and the absence of anti-windup implementations on the physical setup. Our controller tuning keeps the laser input within the desired process window with minimal violations during transients (beginning/end of vector). We experimentally verified that clipping the inputs within a narrow process window band results in excessive lack of fusion. 
\end{itemize}
}

To model the LPBF process, we utilized the dynamical model introduced in \cref{sec:ControlOrientedMultiLayerModel} on the wedge path of \cite{kavas2024situ}, shown in \cref{fig:WedgePath}, which has significant in-layer overheating problems. We treated the following parameters as uncertain: $\alpha$ (absorption), $a$ (laser beam radius), $\epsilon$ (porosity), $k_\text{pd}$ (conductivity between a powder node and the substrate), and $k_\text{p}$ (conductivity between powder nodes).
\jl{The nominal values of the parameters $\theta^{\text{n}}$, listed in \cref{Tab:ProcessParametersReal,Tab:ProcessParametersRealCalibration} in \ref{sec:ModelParametersForSimulationAndExperiments}, were obtained through a calibration process by running a grid search on the intervals described in \cref{tab:grid_search} and choosing the combination of parameters that minimized the cost function
% \begin{align*}
% \mathcal{C}_\text{calibration} (\theta) = \| y_\text{real} - y(\theta) \|_2^2,
% \end{align*}
\begin{align*}
\theta^{\text{n}} = \argmin_{\theta \in \Theta_\text{grid}}\| y_\text{real} - y(\theta) \|_2^2,
\end{align*}
where $\Theta_{\text{grid}}$ denotes the set of all possible combination of parameters from \cref{tab:grid_search},}
$y_\text{real}$ is the output in millivolt obtained from the LPBF machine by applying a constant power of $150\,\si{\watt}$, and $y(\theta)$ is the simulated output obtained with parameters $\theta$, where $\theta=[\alpha,a,\epsilon,k_\text{pd},k_\text{p}]^\top$, with the same constant input.
Note that $y_\text{real}$ is simply \emph{the laser exposure of a single layer of the wedge print during the nominal uncontrolled case}, highlighting the lightweight data requirements of the proposed framework and promoting its utility in practice. 
% \lyg{I don't think we need the italic.}\rz{This is the point we want to stress, should we remove italic or not?}
\begin{table}[H]
\small
\caption{Uncertain parameters and the interval used in the grid search.}\label{tab:grid_search}
\centering
\begin{tabular}{ c c c c}
\toprule
\textbf{Parameter} & \textbf{Description} & \textbf{Interval} & \textbf{Number of Samples} \\
\midrule
$\alpha$        & Fraction of the laser power absorbed by the material & $[0.5,1]$ & 6 \\
$a$             & Cross-section radius of the laser beam & $[4,9] \cdot 10^{-4}$ & 6 \\
$\epsilon$      & Porosity of the metal & $[0.4,0.6]$ & 5 \\
$k_\text{pd}$   & Thermal conductivity between powder and solidified metal & $[0.67, 1.5]$ & 6 \\
$k_\text{p}$    & Thermal conductivity of powder & $[0.5, 5]$ & 10  \\
\bottomrule
\end{tabular}
\end{table}


\eb{To use the model with the measured sensor values, we apply another affine transformation to the simulation outputs.} The units of the output of the simulation are Kelvin. We solve the following linear regression to map simulated signals in Kelvin to the real signals in millivolts
\begin{align*}
y(\theta^{\text{n}}) = \argmin_{A,b} \| y_\text{real} - Ay_{\text{K}}(\theta^{\text{n}}) - b \|_2^2,
\end{align*}
where $y_\text{K}(\theta^{\text{n}})$ is the simulation output in Kelvin using the nominal parameters. \eb{We perform the parameter search over the $\Theta_{\text{grid}}$ while performing the affine transformation map to find the best performing parameter and transform combination in terms of the 2-normed error.}
The simulated \eb{(using the best parameters from the grid search)} and real outputs are shown in Figure \ref{fig:SimRealSimilarity}. 

% \lyg{I don’t understand how this works. 
% You do a different fit of A and b for each $\theta$? Then minimise over $\theta$ above? Why not just add the sensor calibration parameters to A and b to $\theta$ and do the minimisation once? Much simpler to explain, more intuitive, and probably easier to implement. Since we robustify against $\theta$ uncertainty we can just say “we keep A and b constant from now on”.
% If first you fit A, b then the rest please move this part earlier, “for each parameter value $\theta$ we start by calibrating the sensor by solving … We then fit the parameters by minimising …”. 
% How was this bilevel optimisation even implemented?
% What does ‘best observed parameters’ mean? The final parameters you get after this double minimisation?}
% \rz{We mention that this is solved by grid search, so that explains how we solve this bilevel problem. Should we rephrase somehow?}\jl{I changed the formula at the top of this page to make it clearer.}\eb{I think the confusion is partially due to notation. There are two different things and we should signify them with the notation. Please check my updates to confirm.}



\begin{figure}
     \centering
     \input{graphics/tex/wedge_path_new.tex}
     \caption{Wedge path for the laser. The laser scans from right to left, with hatching proceeding from top to bottom.}\label{fig:WedgePath}
\end{figure}

\begin{figure}
     \centering
     \input{graphics/tex/wedge_sim_real_fit.tex}\\
     \caption{Simulation output $y(\theta)$ (orange) and real output $y_\text{real}$ (blue) for the wedge path of \cref{fig:WedgePath} and a constant input of $150\si{\watt}$.} \label{fig:SimRealSimilarity}
\end{figure}

The training of the feedback gains is done in simulation similar to what was done in Section \ref{sec:TrainingSettingForInLayerControlLoop}, but in \cref{eqn:InLayerOptimization} the input is chosen as $u_1[t] = u_1^f[t]+u_1^b[t]$ without any projection $\Pi_{U}$, due to experimental considerations outlined above.
% as the LPBF setup's software does not support real-time projections of the input value.
In addition, the objective function is changed to
\begin{equation}
J_{\text{in}}(K) = \frac{1}{t_p} \mathbb{E}_{w,\theta'} \Bigl[\sum_{j=1}^{t_p} \norm{y_1[j] - y_d}^2 + \lambda P_\text{cst}(u_1) + \eta P_\text{osc}(u_1) \Bigr]%
\label{eq:cost_nominal}
\end{equation}
where $P_\text{cst}$ and $P_\text{osc}$ are input constraint violation and input rate penalties
\begin{align*}
P_\text{cst}(u_1) &= \sum_{j=0}^{t_p-1} \bigl[u_{\text{min}}-u_1[j] \bigl]_+ + \bigl[u_1[j]-u_{\text{max}} \bigl]_+,\\
P_\text{osc}(u_1) &= \sum_{j=1}^{t_p-2} u_1[j-1] - 2 u_1[j] + u_1[j+1]
\end{align*}
where $[x]_+ = \operatorname{max}(0,x)$ and $\lambda$ and $\eta$ are penalty weight factors.
By introducing the penalty $P_\text{cst}$ in the cost function, we encourage the input to remain within the interval $[u_\text{min}, u_\text{max}]$, preventing lack of fusion (when the input drops below $u_\text{min}$) and keyholing (when it exceeds $u_\text{max}$).
The input rate penalty $P_\text{osc}$ discourages large input variations between successive time-steps, thus reducing the aggressiveness of the control action.

Limited by the capability of the physical system, we additionally make the following simplifications on the experimental study: (1) the layer-to-layer control loop produces a single feedforward input that remains constant throughout the entire layer, that is, $u_N^f[t]=u^f$ for all $t=0,\dots,t_p-1$, (2) the in-layer control loop is substituted by a proportional-integral (PI) controller of the form
\begin{equation*}
    u_{N}^b[t]=K_{p} e_{N}[t] + K_i \Delta t \sum_{i=0}^{t} e_{N}[i],
    %\label{eqn:PIController}
\end{equation*}
and the integral term is only accumulated for vectors where the laser is on. 
The full input is therefore given by
\begin{equation*}
    u_{N}[t] = u^f + u_N^b[t]. \\
    % \label{eqn:FullInputReal}
\end{equation*}
%
With these simplifications, our controller becomes a PI controller with a feedforward term, as previously studied in the literature \cite{craeghs2010feedback, shkoruta2022real,kavas2024situ}. Unlike these works, however, \emph{here the tuning is performed in simulation, requiring only the data of a single-layer laser exposure on the real machine for calibration, thus significantly reducing costs.}

The overall tuning problem is summarized in \cref{eq:wedge_design_problem}.
\begin{equation}
\begin{aligned}
    \operatorname*{minimize}_{K,u^f} \quad &J_{\text{in}}(K) = \frac{1}{t_p} \mathbb{E}_{w,\theta'} \Bigl[\sum_{j=1}^{t_p} \norm{y_1[j] - y_d}^2 + \lambda P_\text{cst}(u_1) + \eta P_\text{osc}(u_1) \Bigr] \\
    \text{subject to} \quad &y_1 = Y_{1}^u(\theta') u_1 + Y_{1}^x(\theta') X_1[0] + Y_{1}^d(\theta') \bar{d}_1(\theta'),\\
    &\hat{y}_1[t] = y_1[t] + w[t], \\
    &w[t] \sim \text{Uniform}[w_{\text{min}}, w_{\text{max}}],\\
    &\theta' \sim \text{Uniform}[\theta_{\text{min}}, \theta_{\text{max}}],\\
    &u_1[t] = u^f+u_1^b[t], ~t=0,1,...,t_p-1,\\
    &u_1^b[t]= K_{p} e_{N}[t] + K_i \Delta t \sum_{i=0}^{t} e_{N}[i], ~t=0,1,...,t_p-1,\\
    &e_{1}[i] = y_{1}[i] - \hat{y}_1[i],~i=0,1,\dots,t,\\
    &X_1[0] = \bar{X}_1[0].
    \label{eq:wedge_design_problem}
\end{aligned}
\end{equation}

We trained the proportional gain $K_p$, integral gain $K_i$, and the feedforward term $u^f$ by gradient descent, sampling in each iteration a value for $\theta'=\operatorname{diag}(1+e_\theta)\theta_\text{n}$, where $\theta_\text{n}$ is the nominal value and $e_\theta$ is sampled component-wise uniformly at random from the interval $[-0.05, 0.05]$. 
Moreover, the measurement noise is sampled uniformly at random at each time-step from the interval $[-5,5]$. 
We used the Adam optimizer with $\beta_1=0$, $\beta_2=0.8$ for $200$ iterations. The learning rates are $\gamma=4 \cdot 10^{-3}, 5 \cdot 10^{-4}$ and $2$ for $K_p, K_i$ and $u^f_N[0]$ respectively.
The desired output $y_d$ (in Kelvin) is obtained by converting the desired output signal of \SI{80}{\milli\volt} to Kelvin using the $A$ and $b$ parameters obtained through linear regression.

\subsection{Simulation Setup} \label{sec:experiment_design:simulation}

% \lyg{3.4.1 seems out of place. I would start with what is now 3.4.2 where we talk about how the model was calibrated etc. then come to how the model was used in simulation to train the controller.}
% \rz{I agree but we converged to this structure after deciding to submit to AM.}
Motivated by practical considerations, we assume that the fraction of power absorbed by the material $\alpha$, 
the porosity of the metal $\epsilon$, and the thermal conductivity between powder and solidified metal $\kappa_\text{pd}$, are subject to uncertainty. 
We assume that the true parameter can be expressed as $\theta= [\alpha(1+e_\alpha), \epsilon(1+e_\epsilon), \kappa_\text{pd}(1+e_{\kappa})]^\top$ for some $e_\alpha$, $e_\epsilon$ and $e_\kappa$ and let the nominal value be $\theta'=[\alpha', \epsilon', \kappa_\text{pd}']^\top$.
Numerical values for the process parameters are given in \cref{Tab:ProcessParameters} in \ref{sec:ModelParametersForSimulationAndExperiments}. 
Both the training and testing of the dual-loop controller are done using the square spiral laser scanning path on the left-hand side of \cref{fig:SquareSpiral}. 
This path is particularly challenging for two reasons: (1) it demonstrates severe overheating problems, 
(2) it requires a relatively aggressive input change in the printing process to stabilize the temperature, 
as shown in the right-hand side of \cref{fig:SquareSpiral}.
% \lyg{Training and testing on the same pattern leaves us open to criticism of overfitting. Can brush it under the rug here, but in principle we should try on other patterns too, say a raster or a spiral or something, to see if the results generalise }

\begin{figure}
\centering
\input{graphics/tex/revised_new_path_and_input_plot.tex}
\caption{Square spiral path for the laser (left), associated optimal input (upper right) and realized output (lower right) for $y_d=1500~\text{K}$ and nominal parameters. Note that at each corner, the laser power should drastically decrease for the best temperature stabilization.}%\eb{Please add the output for this optimal input to the plot}
\label{fig:SquareSpiral}
\end{figure}

\paragraph{Training Setting for In-layer Control Loop}\label{sec:TrainingSettingForInLayerControlLoop}

We train the feedback gain $K$ by solving (\ref{eqn:InLayerOptimization}) using \cref{alg:backprop}. 
For each training iteration, 32 models with uncertain parameters randomly generated from 
$e_\alpha, e_\epsilon, e_\kappa \sim \text{Uniform}[-0.2, 0.2]$ are used to construct the system dynamics. 
The controller is trained for 50 iterations starting with $K=0$ using Adam with learning rate $\gamma=2 \cdot 10^{-3}$ and $\beta_1=0$, $\beta_2=0.8$ (parameters obtained through manual tuning).
The entire training procedure takes approximately 3 minutes on a NVIDIA GeForce RTX 3050 Ti GPU. 
The measurement noise $w \sim \text{Uniform}[\SI{-10}{\kelvin},\SI{10}{\kelvin}]$ is drawn randomly at each time
step to improve the robustness of the in-layer controller. 
The desired temperature is set to $y_d=\SI{1500}{\kelvin}$.

\subsection{Experiment plan}

We performed five experiments in total. 
For three of them we used controllers obtained by solving \cref{eq:wedge_design_problem} with different penalty parameters, specifically i) $\lambda=30$, $\eta = 15 $, ii) $\lambda=50$, $\eta = 50 $, and iii) $\lambda=125$, $\eta=0$ (i.e., no rate penalization). 
We further tested the PI controller of \cite{kavas2024situ} (hereafter referred to as Bayesian Optimization (BO)) and additionally a constant input set to $\SI{150}{\watt}$.
The BO controller of \cite{kavas2024situ} was tuned without feedforward static input by minimizing an objective function including a tracking cost to ensure that the output is as close as possible to \SI{80}{\milli\volt} as well as a penalty on the input rate to penalize large input changes in successive time steps.
% \bk{All parts planned are described here (ALL experiments that are planned), with 4 of them specifically shown with the results etc.}
% Five experiments were performed by printing the wedge geometry with the following controller settings:
% \begin{itemize}
%     \item Optimized with penalty ($\lambda=30, \eta = 15 $)
%     \item Optimized with penalty ($\lambda=50, \eta = 50 $)
%     \item Optimized with penalty ($\lambda=125$)
%     \item Bayesian Optimized parameters (legacy)
%     \item Uncontrolled (No closed-loop control)
% \end{itemize}
%

The parts are printed on large cross-sectioned support structures and manually removed from the build platform upon completion.
Each part is printed for 150 layers.
Upon removal, parts have been 3d scanned and pictured in different angles with the Keyence VHX-7000 optical microscope setup.
The microscopic evaluations are carried according to \cref{section:micro_evaluation}.
% They were cut close to their center line by a Struers Accutom-10 cutting machine aligned with layer applicaiton during the printing process to observe the transverse cross-section, then metallographically prepared by embedding, grinding, and polishing.
% Embedding was performed hot by a Struers CitoPress machine with DuroLite bakelite resin grinding with 320-grit sandpaper, and polishing with Struers commercial polishing cloths Largo, Dac, Nap, and Chem with suspensions with particle sizes of $\SI{9}{\micro\meter}$, $\SI{3}{\micro\meter}$, $\SI{1}{\micro\meter}$, and $\SI{0.1}{\micro\meter}$, respectively.
Finally, the polished mounts are inspected in coaxial and ring lighting modes with the microscope to observe the microstructure.
% \rz{Isn't this largely repeating what was previously written in \cref{section:micro_evaluation}?}

==> sections/old_sections/3_dual_loop_control_scheme.tex <==
\section{Dual-loop Control Scheme} \label{Dual-LoopControlScheme}

The control architecture proposed in this paper consists of two nested control loops, illustrated in \cref{fig:SLMControlArchitecture}. The \emph{layer-to-layer control loop} provides optimized feedforward input profiles for an entire layer, while the \emph{in-layer control loop} uses real-time pyrometer measurements to adjust the laser power at run-time as the layer is being printed. The full input is
\begin{equation}
    u_{N}[t] = \Pi_{U} \Bigl(u^f_N[t] + \sum_{k=1}^N u_k^b[t] \Bigl)\text{,} \\
    \label{eqn:FullInput}
\end{equation}
where $u_N^f[t]$ is the feedforward layer-to-layer control for layer $N$, $u_{k}^b[t]$ is the feedback in-layer control for layer $k$, $\Pi_U$ denotes the Euclidean projection onto the set $U=[u_\text{min}, u_\text{max}]$, where $u_{\text{min}}, u_{\text{max}}$ are the minimal and maximal laser power respectively.

The use of a nested control architecture is motivated by the layer-to-layer nature of the SLM process. The outer loop utilizes layer-wide measurements to iteratively correct the feedforward input trajectory, ensuring that the tracking performance improves layer after layer; however, this controller alone does not have any immediate effects within each layer. This motivates the second in-layer control loop, which is able to quickly reduce the tracking error by utilizing online measurements.

We now explain in detail both the control loops, starting with the layer-to-layer part.

\subsection{Layer-to-layer Control Loop Design}\label{sec:LayerToLayerControlLoopDesign}

The layer-to-layer control loop generates feedforward input trajectories $u^f_N$ using measurements $\hat{y}_N$ collected after printing each layer. The controller is formulated as a convex optimization problem combining TTO and ILC. To ensure computational tractability, we only consider single layer dynamics by using (\ref{eqn:LiftedSystem}) as a model with $N=1$. The optimization problem that must be solved after each print is given by
\begin{align}
\begin{split}
\operatorname*{minimize}_{u_N^f} \quad &J_N(u_N^f) = \sum_{j=1}^{t_p} \|{y_N[j] - y_d}\|_{Q}^2 + \|{u_N^f[j-1]}\|_{R}^2 \\
\text{subject to} \quad &y_N = Y_{1}^u(\theta') u_N^f + Y_{1}^x(\theta') X_1[0] + Y_{1}^d(\theta') \bar{d}_1(\theta')\\
& \hphantom{y_N =} + \sum_{k=1}^{N-1} L_y (\hat{y}_{k} - y_{k}),\\
% \text{s.t.} \quad &X_1[l+1] = \Bar{A}_{1}(\theta) X_1[l] + \Bar{B}_{1}(\theta)[l] u_N[l] + \Bar{d}_{1}(\theta)\\
% &y_N[l] = \Bar{C}_{1}(\theta)[l] X_1[l] + \sum_{k=1}^{N-1} L (\Tilde{y}_{k}[l] - y_{k}[l]) \\
% &\Tilde{y}_{0}[l] \equiv 0, ~y_{0}[l] \equiv 0\\
&X_1[0] = T_s\mathbf{1}_n,\\
%&u_N[l] = v_N[l]+\sum_{k=1}^{N-1} \Delta u_{k}[l]\\
&u_{\text{min}} \leq u_N^f[t] \leq u_{\text{max}},~t=0,1,...,t_p-1,
\end{split}\label{eqn:LayerToLayerOptimization}
\end{align}
where $L_y\in(0,2)$ is a learning gain, $u_N^f$ is the feedforward input, $y_N$, $y_d$, and $\hat{y}_k$ are the nominal output for layer $N$, the desired output, and the measured output for layer $k$, respectively. The cost penalizes the output tracking error $y_N[j]-y_d$ as well as the control input, where the matrices $Q$ and $R$, similar to the classic LQR setting, can be tuned to reduce the aggressiveness of the control update (by increasing $R$ compared to $Q$) or to increase the tracking performance (by increasing $Q$). The term $\sum_{k=1}^{N-1} L_y (\hat{y}_{k} - y_{k})$ is used to iteratively correct the error caused by model reduction, incorrect parameter estimation, and measurement noise, using measurement of outputs collected in previous layers. This is similar to the well-known \emph{norm-optimal ILC} \cite{amann1996optimal, NO-ILCwithConstraint}, which is retrieved if $L_y=1$. %\eb{I don't clearly see how this would be the case with model mismatch.}

Problem \eqref{eqn:LayerToLayerOptimization} is a quadratic program (QP) that can be solved efficiently using specialized software. Choosing $z=u_N^f$, we can express \eqref{eqn:LayerToLayerOptimization} in standard form as
\begin{align}
\begin{split}
\operatorname*{minimize}_{z} \quad &\frac{1}{2} z^\top H z + f^\top z \\
\text{subject to} \quad &Gz \leq S,\\
\end{split}\label{eqn:LayerToLayerOptimizationSimplified}
\end{align}
with $H = 2 (\bar{R} + Y_1^u (\theta')^\top \bar{Q} Y_1^u (\theta')$), $f = 2 (\phi - \bar{y}_d)^\top \bar{Q} Y_1^u (\theta')$, $\phi = Y_1^x (\theta') X_1[0] + Y_1^d (\theta') \bar{d}_1 (\theta') + \sum_{k=1}^{N-1} L_y (\hat{y}_k - y_k)$, $G = \operatorname*{col}[I_n, -I_n]$, and $S = \operatorname*{col}[\bar{u}_{\text{max}}, -\bar{u}_{\text{min}}]$, where $\bar{Q}$, $\bar{R}$ are block diagonal matrices and $\bar{y}_d$, $\bar{u}_\text{max}$, $\bar{u}_\text{min}$ are vectors obtained by stacking repeated copies of $Q$, $R$, $y_d$, $u_\text{max}$, and $u_\text{min}$, respectively.

% Let $\bar{Q} = \text{diag}[Q, Q, ..., Q]$, $\bar{R} = \text{diag}[R, R, ..., R]$, $\bar{y}_d = \text{diag}[y_d, y_d, ..., y_d]$, $\bar{u}_{\text{min}} = \text{diag}[u_{\text{min}}, u_{\text{min}}, ..., u_{\text{min}}]$, and $\bar{u}_{\text{max}} = \text{diag}[u_{\text{max}}, u_{\text{max}}, ..., u_{\text{max}}]$.

% , then $y_N^e = Y_1^u (\theta')z + \phi$, where the constant $\phi$ is defined as
% \begin{equation}
%     \phi = Y_1^x (\theta') X_1[0] + Y_1^d (\theta') \bar{d}_1 (\theta') + \sum_{k=1}^{N-1} L_y (\hat{y}_k - y_k^e).
%     \label{eqn:DefinitionPhi}
% \end{equation}

% \textcolor{red}{Note that in order to implement an NO-ILC-like layer-to-layer control, $\sum_{k=1}^{N-1} \Delta u_{k}[l]$ is added in addition to $\Delta u_{N}[l]$ to form the full input in (\ref{eqn:FullInput}) since $\Tilde{y}_{k}$ is derived with $\Delta u_{k}[l]$ coming into play for all $k\leq N-1$.}

% A zero-phase first-order Butterworth filter \cite{zero-phaseFilter}, whose critical frequency is half of the Nyquist frequency, is applied to transform $\hat{y}_k$ to $\Tilde{y}_{k}$ from $l=5$, with  $\Tilde{y}_{k}[l]=\hat{y}_k[l]$ for $k=0,1,2,3,4$. The transfer function of the filter in the z-domain is expressed as
% \begin{equation}
%     H(z) = 0.5+0.5z^{-1}
%     \label{eqn:ZeroPhaseFilter}
% \end{equation}

% The summations in the constraints of TTO and in the (\ref{eqn:FullInput}) can be easily turned into a recursive representation. By leveraging the output history and additional feedback input history in a recursive way, which is the core idea of ILC, TTO can improve its tracking performance under model mismatch and measurement noise without using the multi-layer model.

\subsection{In-layer Control Loop Design}\label{sec:InLayerControlLoopDesign}

The in-layer control loop uses real-time output measurement $\hat{y}_N[t]$, collected as the layer is being printed, to adjust the laser power, enabling real-time feedback. The feedback term $u_N^b[t]$ is given by the following linear output disturbance feedback scheme
\begin{equation}
    u_{N}^b[t]=\sum_{i=0}^{t} K_{t}[i] e_{N}[i]\text{,}
    \label{eqn:DisturbanceFeedback}
\end{equation}
where $K_{t}[i]$ is a feedback gain and $e_{N}[i] = y_{N}[i] - \hat{y}_N[i]$. The gains $K_t[i]$ must be determined offline before starting the print of the first layer. To obtain them, we solve the following optimization problem, where $K$ is the matrix with $K_t[i]$ on its $t$-th row and $i$-th column:
\begin{equation}
\begin{aligned}
    \operatorname*{minimize}_K \quad &J_{\text{in}}(K) = \mathbb{E}_{w,\theta'} \Bigl[~\frac{1}{t_p} \sum_{j=1}^{t_p} \norm{y_1[j] - y_d}^2~\Bigl] \\
    \text{subject to} \quad &y_1 = Y_{1}^u(\theta') u_1 + Y_{1}^x(\theta') X_1[0] + Y_{1}^d(\theta') \bar{d}_1(\theta'),\\
    &\hat{y}_1[t] = y_1[t] + w[t], \\
    &w[t] \sim \text{Uniform}[w_{\text{min}}, w_{\text{max}}],\\
    &\theta' \sim \text{Uniform}[\theta_{\text{min}}, \theta_{\text{max}}],\\
    &u_1[t] = \Pi_U \Bigl(u_1^f[t]+u_1^b[t] \Bigl),\\
    &u_1^b[t]=\sum_{i=0}^{t} K_{t}[i] e_{1}[i], ~t=0,1,...,t_p-1,\\
    &e_{1}[i] = y_{1}[i] - \hat{y}_1[i],~i=0,1,\dots,t,\\
    &X_1[0] = \bar{X}_1[0],
    \label{eqn:InLayerOptimization}
\end{aligned}
\end{equation}
where $y_1, \hat{y}_1$ represent the true measured outputs for a given layer, $w_{\text{min}}, w_{\text{max}}$ denote the bounds on the measurement noise, $\theta'_{\text{min}}, \theta'_{\text{max}}$ are the minimal and maximal parameter estimates, $u_1^f$ is the feedforward input given by the layer-to-layer controller by solving \cref{eqn:LayerToLayerOptimization} for layer $1$, and $\bar{X}_1[0]$ is an estimate for the initial state of the system. Since \cref{eqn:InLayerOptimization} considers the initial layer only, we set $X_1[0] = T_s\mathbf{1}_n$, as initially the powder is at the same temperature as the build plate.

By explicitly accounting for model uncertainty and noise in \cref{eqn:InLayerOptimization}, we ensure that any minimizer $K$ of the problem is robust when deployed in closed-loop operation.

To solve \cref{eqn:InLayerOptimization} efficiently, we apply a gradient-based scheme to an unconstrained reformulation of \cref{eqn:InLayerOptimization}. For a given value of $w$ and $\theta'$, the gradient of the loss function $J_{\text{in}}(K)$ is given by
\begin{equation}
    \nabla J_{\text{in}}(K) = \frac{\partial J_{\text{in}}(K)}{\partial y_1} \frac{\partial y_1}{\partial u_1} \frac{\partial u_1}{\partial u_1^b} \frac{\partial u_1^b}{\partial K},
    \label{eqn:FullGradient}
\end{equation}
where $\partial J_{\text{in}}(K)/\partial y_1 = \operatorname*{sign}(y_1-y_d) / t_p$, $\partial y_1/\partial u_1 = Y_{1}^u(\theta')$, $\partial u_1/\partial u_1^b = \text{diag} ( \text{sat}(u_1^f+u_1^b) )$, with $\operatorname*{sat}(u)=1$ if $u\in U$ and $\operatorname*{sat}(u)=0$ otherwise, and $\partial u_1^b/\partial K$ is given by \jl{I am confused with this expression, not sure if it is correct or not}
\begin{align*}
\frac{\partial u_1^b}{\partial K_t} = - \mathds{1}_t \otimes w^\top,
\end{align*}
for each $t$, where $\otimes$ denotes the kronecker product and $\mathds{1}_t$ is the vector containing a one in its $t$-th row and $0$ elsewhere. In \cref{SimulationExperiments}, we evaluate the derivative in \cref{eqn:FullGradient} using efficient automatic differentiation tools.

To solve \cref{eqn:InLayerOptimization}, we randomly sample elements of $w$ and $\theta'$, evaluate \cref{eqn:FullGradient} and implement a single gradient step of the form
\begin{align*}
K^{k+1} = K^k - \alpha_k \nabla J_\text{in}(K^k),
\end{align*}
where $K^{k+1}$ and $K^k$ denotes the updated and the starting value of the control matrix, respectively, $\alpha_k>0$ is a stepsize, and $k\in \mathbb{N}$ is an iteration index. Pseudo code to solve \cref{eqn:InLayerOptimization} is summarized in \cref{alg:backprop}. \jl{Since I used Adam (with momentum), the gradient descent is actually not implemented in the way above. Should we change it?}

\begin{algorithm}
\caption{Gradient-based algorithm to solve \cref{eqn:InLayerOptimization}} \label{alg:backprop}
\begin{algorithmic}
\State \textbf{Require:} $K^0$, $\{ \alpha_k \}_{k\in \mathbb{N}} \subset \R_{>0}$.
\State \textbf{Init:} $k\gets 0$
\While{\texttt{not\_terminated}}
    \State Sample $w[t] \sim \operatorname*{Uniform}[w_\text{min},w_\text{max}]$ for $t=1,\dots,t_p$.
    \State Sample $\theta'\sim \operatorname*{Uniform}[\theta_\text{min},\theta_\text{max}]$.
    \State Compute gradient $\nabla J_\text{in}(K^k)$ using \cref{eqn:FullGradient}.
    \State Update $K^{k+1}=K^k-\alpha_k \nabla J_\text{in}(K^k)$.
    \State $k\gets k+1$
\EndWhile
\State \textbf{Return:} $K^{k}$
\end{algorithmic}
\end{algorithm}

Under mild conditions on the stepsizes, the following holds.

\begin{theorem}\label{thm:main}
Suppose $\alpha_k$ is square summable but not summable. Then the \cref{alg:backprop} converges asymptotically to a critical point of \cref{eqn:InLayerOptimization}.
\end{theorem}
%
\begin{proof}
Each expression in \cref{eqn:FullGradient} belongs to the class of functions definable in an o-minimal structure \cite{coste1999introduction}. As a result, the stochastic gradient descent scheme in \cref{alg:backprop} converges to a critical point by \cite[Theorem 2]{davis2020stochastic}.
\end{proof}

% \subsection{In-layer Control Loop Design with Output Constraints}\label{sec:InLayerControlLoopDesignWithSoftOutputConstraint}

% The control gains can also be selected to ensure output constraint satisfaction. We consider constraints of the form
% \begin{equation}
%     y_d-\rho \leq y_1[l] \leq y_d+\rho
%     \label{eqn:OutputConstraintFormulation}
% \end{equation}
% for some $\rho > 0$ and all $l\geq3$. We enforce Inequality (\ref{eqn:OutputConstraintFormulation}) using the penalty function
% \begin{equation}
%     f(\rho, K) = a_\rho \norm{\rho_{\text{up},1} + \rho_{\text{low},1}}_2
%     \label{eqn:OutputPenalty}
% \end{equation}
% where
% \begin{equation}
% \begin{aligned}
%     \rho_{\text{up},1} = \Bigl[&\max{\Bigl(y_1[3]-(y_d+\rho), 0\Bigl)}, ..., \\
%     &\max{\Bigl(y_1[l_p]-(y_d+\rho), 0\Bigl)}\Bigl]^T\\
%     \rho_{\text{low},1} = \Bigl[&\max{\Bigl((y_d-\rho)-y_1[3], 0\Bigl)}, ..., \\
%     &\max{\Bigl((y_d-\rho)-y_1[l_p], 0\Bigl)}\Bigl]^T\\
%     \label{eqn:OutputPenaltyTermClarification}
% \end{aligned}
% \end{equation}
% The coefficient $a_\rho$ is used to balance the inexact tracking cost and the output constraint violation cost. We choose to use the 2-norm $\norm{\cdot}_2$ in the penalty function to ensure the smoothness of the objective, and the calculation of constraint violation starts from time step $l=3$ to allow the temperature to increase to the neighborhood of the desired temperature in the first few time steps.

% The resulting optimization problem is
% \begin{equation}
% \begin{aligned}
%     \argmin_K \quad &J_{\text{in}}^{\rho}(K) = \mathbb{E}_{w,\theta'} \Bigl[~\frac{1}{l_p} \sum_{j=1}^{l_p} \norm{y_1[j] - y_d}~ + f(\rho, K)\Bigl] \\
%     \text{s.t.} \quad &y_1 = Y_{1}^u(\theta') u_1 + Y_{1}^x(\theta') X_1[0] + Y_{1}^d(\theta') \bar{d}_1(\theta') \\
%     &\hat{y}_1[l] = y_1[l] + w[l] \\
%     &w[l] \sim U[w_{\text{min}}, w_{\text{max}}] \\
%     &\theta' \sim p(\theta')\\
%     &X_1[0] = T_s\mathbf{1}_n\\
%     &u_1[l] = \Pi_U \Bigl(u_1^e[l]+\Delta u_1[l] \Bigl)\\
%     &\Delta u_1[l]=\sum_{i=0}^{l} K_{l}[i] e_{1}[i],~l=0,1,...,l_p-1\\
%     &e_{1}[i] = y_{1}^e[i] - \hat{y}_1[i]\\
%     \label{eqn:InLayerOptimizationRho}
% \end{aligned}
% \end{equation}
 
% In \cref{SimulationExperiments}, we show how (\ref{eqn:InLayerOptimization}) can be solved efficiently using a gradient descent scheme. %
% to optimize $K$ in  to obtain control gains that are robust to model mismatche and measurement noise. 
% This idea has been investigated in \cite{GD-OutputFeedback}.
% To reduce the computation time necessary to complete the tuning, we restrict the gain optimization to a single layer.

==> sections/old_sections/4_simulation_experiments.tex <==
% \subsection{Simulation Experiments} \label{SimulationExperiments}

% In this section, we train and deploy the dual-loop scheme introduced in \cref{Dual-LoopControlScheme} on a simulated SLM machine. The detailed procedure is shown in Figure \ref{fig:AlgorithmDiagram}. Motivated by practical considerations, we assume that the fraction of power absorbed by the material $\alpha$, the porosity of the metal $\epsilon$, and the thermal conductivity between powder and solidified metal $\kappa_{pd}$, are subject to uncertainty. Specifically, we let $\theta=[\alpha, \epsilon, \kappa_{pd}]^T$ and $\theta'=[\alpha', \epsilon', \kappa_{pd}']^T$ with 
% \begin{equation}
%     \theta' = \operatorname*{diag}(1+e_\alpha, 1+e_\epsilon, 1+e_{\kappa}) \theta,
% %     \begin{bmatrix}
% %     1+e_\alpha & & \\
% %      & 1+e_\epsilon & \\
% %      & & 1+e_{\kappa}\\
% %     \end{bmatrix} \theta\text{,}
%     \label{eqn:UncertaintyRelation}
% \end{equation}
% where $e_\alpha$, $e_\epsilon$ and $e_\kappa$ represent the estimation error. Numerical values for the process parameters are given in \cref{Tab:ProcessParameters} in \cref{sec:ModelParametersForSimulation}.

% Unless otherwise stated, both the training and testing of the dual-loop controller use the square spiral laser scanning path in the left-hand side of \cref{fig:SquareSpiral}. This path is particularly challenging for two reasons: (1) it demonstrates severe overheating problems, (2) it requires a relatively aggressive input change in printing process to stabilize the temperature, as shown in the right-hand side of \cref{fig:SquareSpiral}.

% \begin{figure}
% % \begin{subfigure}[t]{.5\columnwidth}
% %   \centering
% %   \input{graphics/tex/path.tex}
% % %   \vspace{-10pt}
% % %   \caption{Square spiral path for the laser.}
% % %   \label{fig:SquareSpiral}
% % \end{subfigure}%
% % \begin{subfigure}[t]{.5\columnwidth}
% %   \centering
% %   \input{graphics/tex/best_input.tex}
% % %   \vspace{2pt}
% % %   \caption{1b}
% % %   \label{fig:sfig2}
% % \end{subfigure}
% \centering
% \input{graphics/tex/revised_new_path_and_input_plot.tex}
% \caption{Square spiral path for the laser (left), and associated optimal input for $y_d=1500~\text{K}$ and nominal parameters. Note that at each corner, the laser power should drastically decrease for the best temperature stabilization.}
% \label{fig:SquareSpiral}
% \end{figure}
% %
% % \begin{figure}
% %      \centering
% %      \input{graphics/tex/path.tex}
% %      % \includegraphics[width=0.45\textwidth]{graphics/square_spiral_new.pdf}\\
% %      \caption{Square spiral path for the laser.}\label{fig:SquareSpiral}
% % \end{figure}
% % \begin{figure}
% %      \centering
% %      % \captionsetup{skip=-3pt}
% %      % \includegraphics[width=.445\textwidth]{graphics/perfect_tracking_input_new.pdf}
% %      \input{graphics/tex/best_input.tex}
% %      \caption{Input for layer 1 that realizes perfect temperature tracking with $y_d=1500~\text{K}$ and nominal parameters. Note that at each corner, the laser power should drastically decrease for the best temperature stabilization.}\label{fig:PerfectTrackingInput}
% % \end{figure}

% \subsection{Training Setting for In-layer Control Loop}\label{sec:TrainingSettingForInLayerControlLoop}

% We train the feedback gain $K$ by solving (\ref{eqn:InLayerOptimization}) using gradient descent leveraging the automatic differentiation tools of Pytorch \cite{paszke2019pytorch}. The batch size is 32 and, for each training epoch, 32 models with uncertain parameters randomly generated from $e_\alpha, e_\epsilon, e_\kappa \sim \text{Uniform}[-0.2, 0.2]$ are used to construct the system dynamics, while the layer-to-layer controller utilizes the model with nominal parameters. The controller is trained for 50 epochs starting with $K=\mathbf{0}$ and using Adam \cite{kingma2014adam}. Adam does not posses the convergence guarantees of \cref{thm:main}; nevertheless, it showed superior performance compared to standard stochastic gradient descent for our problem. The entire training procedure takes approximately 3 minutes on a NVIDIA GeForce RTX 3050 Ti GPU. The measurement noise $w \sim \text{Uniform}[\SI{-10}{\kelvin},\SI{10}{\kelvin}]$ is drawn randomly at each time step to improve the robustness of the in-layer controller. For the desired temperature, we consider $y_d=\SI{1500}{\kelvin}$.

% \subsection{Testing Setting for Dual-loop Control Scheme}\label{sec:TestingSettingForDualLoopControlScheme}
% We test the performance of the dual-loop controller by simulating the SLM process for 6 layers. The testing models are also subject to uncertainty $e_\alpha, e_\epsilon, e_\kappa$ taken from $S_e=$\{-0.2, -0.15, -0.1, -0.05, 0, 0.05, 0.1, 0.15, 0.2\}, and there are in total $9^3=729$ possible combinations of testing parameters.
% % whereas the training process only considered $16\times15=240$ possible models. 

% We simulate the SLM process with measurement noise $w\sim\text{Uniform}[\SI{-10}{\kelvin},\SI{10}{\kelvin}]$. 
% % In this case, we filter the measured output $\hat{y}_k$ using a Butterworth filter \cite{zero-phaseFilter}, with critical frequency equal to half of the Nyquist frequency. Next, we consider a noise-free setting to demonstrate that, in absence of noise, our scheme converges to the desired temperature asymptotically.
% %
% % test both with and without measurement noise. In the former case, we choose $w \sim \text{Uniform}[-10~\text{K}, 10~\text{K}]$ and showcase that our scheme maintains robustness; in the latter, we show that convergence to optimal temperature is achieved.
% %
% Additionally, we compare our dual-loop controller with both a single-loop in-layer controller (where $u_N^f[l] \equiv u_1^f[l]$ for all $N$ and $l$, and the full input is chosen as $u_N[l] = u_1^f[l]+ u_{N}^b[l]$) and a single-loop layer-to-layer controller without any in-layer feedback (where $K=\mathbf{0}$ and the full input is $u_N[l]=u_N^f[l]$).
% % , and we compare the dual-loop controller considering output constraints with that not considering output constraints in Section \ref{subsec:DualLoopControlWithOutputConstraint}.

\subsection{Simulation Results}\label{sec:SimulationResults}

% \subsection{Dual-loop Control without Output Constraint}\label{subsec:DualLoopControlWithoutOutputConstraint}

Figures \ref{fig:MeanAE3controllers} show the mean absolute error $\text{MeanAE}_k$ of different controllers across different iterations, where
%
\begin{equation*}
    \text{MeanAE}_k = \frac{1}{t_p-2}\sum_{j=3}^{t_p} \norm{y_k[j] - y_d}.
    %\label{eqn:MeanAE}
\end{equation*}

\begin{figure}
     \centering
     % \includegraphics[width=0.45\textwidth]{graphics/MeanAE_3controllers_new.pdf}
     % \includegraphics[width=0.45\textwidth]{graphics/MeanAE_3controllers_no_noise_new.pdf}
     % \input{graphics/tex/fig6_upper.tex}
     % \vskip 0pt
     % \input{graphics/tex/fig6_lower.tex}
     % \vskip -3pt
     \input{graphics/tex/MeanAE_3controllers_new.tex}
     \vskip -3pt
     \caption{Box plots of the mean absolute error for each controller with measurement noise. The lower quartiles of layer 1 and 2 for layer-to-layer controller are $\SI{45.7}{\kelvin}$ and $\SI{31.8}{\kelvin}$ respectively.}
     \label{fig:MeanAE3controllers}
\end{figure}

\begin{figure}
     \centering
     \input{graphics/tex/dual_loop_box_plot_new.tex}
     \vskip -3pt
     \caption{Upper and lower bounds of all tested outputs obtained with the dual-loop controller with measurement noise.}
     \label{fig:Envelope}
\end{figure}

% \begin{figure}
%      \centering
%      % \includegraphics[width=0.45\textwidth]{graphics/MaxAE_3controllers_new.pdf}
%      % \vskip 5pt
%      % \includegraphics[width=0.45\textwidth]{graphics/MaxAE_3controllers_no_noise_new.pdf}
%      \input{graphics/tex/fig7_upper.tex}
%      \vskip 0pt
%      \input{graphics/tex/fig7_lower.tex}
%      \vskip -3pt
%      \caption{Box plots of the maximum absolute error for each controller with (upper) and without (lower) measurement noise. Note that some data do not scale well with the plot and their values are presented in \cref{Tab:MaxAEPercentile}.}
%      \label{fig:MaxAE3controllers}
% \end{figure}

% \begin{table}[htbp]
%     \renewcommand{\arraystretch}{1.2} % Adjust row spacing
%     \caption{Percentile values of the mean absolute error for the layer-to-layer controller across six layers}
%     \centering
%     \begin{tabularx}{\columnwidth}{|c| *{5}{>{\centering\arraybackslash}X|}}
%         \hline
%         \multirow{2}{*}{Layer} & \multicolumn{5}{c|}{Percentile (with/without measurement noise)}\\ \cline{2-6}
%         & 0\% & 25\% & 50\% & 75\% & 100\% \\ 
%         \hline
%         1 & 1.1/0.9 & 44.7/44.4 & 92.4/93.2 & 157/157 & 408/409\\
%         \hline
%         2 & 11.1/10.7 & 16.1/16.0 & 19.5/20.0 & 26.4/26.0 & 132/133\\
%         \hline
%         3 & 8.4/7.6 & 11.4/11.3 & 13.3/13.1 & 15.3/15.2 & 56.2/58.3\\
%         \hline
%         4 & 4.1/1.6  & 13.0/13.5 & 15.6/16.4 & 18.6/19.5 & 24.2/24.1\\
%         \hline
%         5 & 12.4/13.6  & 17.6/18.5 & 22.7/23.6 & 26.6/27.6 & 31.6/32.4\\
%         \hline
%         6 & 7.7/8.1 & 15.9/16.7 & 20.9/21.9 & 26.0/27.1 & 33.2/34.8\\
%         \hline
%     \end{tabularx}
%     \label{Tab:MeanAEPercentile}
% \end{table}

% \begin{table}[htbp]
%     \renewcommand{\arraystretch}{1.2} % Adjust row spacing
%     \caption{Percentile values of the maximum absolute error for the layer-to-layer controller across first two layers}
%     \centering
%     \begin{tabularx}{\columnwidth}{|c| *{5}{>{\centering\arraybackslash}X|}}
%         \hline
%         \multirow{2}{*}{Layer} & \multicolumn{5}{c|}{Percentile (with/without measurement noise)}\\ \cline{2-6}
%         & 0\% & 25\% & 50\% & 75\% & 100\% \\ 
%         \hline
%         1 & 2.9/1.3 & 53.8/54.0 & 100/100 & 161/162 & 413/414\\
%         \hline
%         2 & 27.0/28.2 & 50.6/48.8 & 62.0/62.4 & 73.7/74.4 & 153/146\\
%         \hline
%     \end{tabularx}
%     \label{Tab:MaxAEPercentile}
% \end{table}

We choose $j=3$ as starting time in $\text{MeanAE}_k$ because heating the powder layer from \SI{900}{\kelvin} to \SI{1500}{\kelvin} requires several time steps even when applying the maximal laser input. As a result, including the first few time steps in the statistics would raise the baseline error equally for all controllers, and therefore visually reduce the gap between the control performances of different controllers.

The figure shows that the dual-loop controller outperforms the other two single-loop controllers. Specifically, while the in-layer controller initially performs well, its mean absolute error shows an upward trend as more layers are printed, indicating that this control architecture alone struggles to maintain accuracy when heat starts accumulating across layers.

Figure \ref{fig:Envelope} shows the upper and lower bounds of all tested outputs obtained with the dual-loop controller. It shows that even at the beginning of the printing process in each layer, the output curve converges to a neighborhood of desired output, despite the presence of measurement noise. 
% When the measurement noise is absent, the tracking improves greatly.

% \begin{figure}
%      \centering
%      % \includegraphics[width=0.45\textwidth]{graphics/envelope_plot_new.pdf}
%      % \vskip -25pt
%      % \includegraphics[width=0.45\textwidth]{graphics/envelope_plot_no_noise_new.pdf}
%      % \vskip -3pt
%      \input{graphics/tex/fig8_upper.tex}
%      \vskip 5pt
%      \input{graphics/tex/fig8_lower.tex}
%      \caption{Upper and lower bounds of all tested outputs obtained with the dual-loop controller with (upper) and without (lower) measurement noise.}
%      \label{fig:Envelope}
% \end{figure}

% To further test the robustness of the controller, we deploy the dual-loop controller on systems with uncertainty on parameters that are considered certain during training. The results are summarized in Figure \ref{fig:Unexpected}, in which all controllers are tested with uncertainties in the fraction of power absorbed by the material $\alpha$, the porosity of the metal $\epsilon$, and the thermal conductivity between powder and solidified metal $\kappa_{pd}$, but dual-loop-$\alpha$ and dual-loop-$\epsilon$ are trained with uncertainty only in $\alpha$ and $\epsilon$ respectively. One can see that the overall performances of all the controllers are similar, suggesting the controller is robust against unexpected uncertain models.

% \begin{figure}
% %     \vskip -28pt
%      \centering
%      % \includegraphics[width=0.45\textwidth]{graphics/MeanAE_unexpected_new.pdf}
%      \input{graphics/tex/fig9_upper.tex}
%      % \vskip -25pt
%      % \includegraphics[width=0.45\textwidth]{graphics/MaxAE_unexpected_new.pdf}
%      \input{graphics/tex/fig9_lower.tex}
%      % \vskip -3pt
%      \caption{Box plots of mean absolute error (upper) and maximum absolute error (lower) given by each controller without measurement noise. "dual-loop-$\alpha$" and "dual-loop-$\epsilon$" are the controllers that are trained with only uncertain $\alpha$ and $\epsilon$ respectively.}
%      \label{fig:Unexpected}
% \end{figure}

% Figure \ref{fig:Envelope1200K} shows that even when $y_d$ changes from \SI{1500}{\kelvin} to \SI{1200}{\kelvin}, the controller is still able to drive the temperature to the desired one despite having been trained with $y_d=\SI{1500}{\kelvin}$.

% \begin{figure}
%      \centering
%      % \captionsetup{skip=0pt}
%      % \includegraphics[width=.45\textwidth]{graphics/envelope_plot_no_noise_1200K_new.pdf}
%      \input{graphics/tex/fig10_lower.tex}
%      \caption{Upper and lower bounds of all tested outputs derived by the dual-loop controller without measurement noise. $y_d=\SI{1200}{\kelvin}$. Note that the controller is trained with $y_d=\SI{1500}{\kelvin}$.}\label{fig:Envelope1200K}
% \end{figure}

% \subsection{Dual-loop Control with Output Constraint}\label{subsec:DualLoopControlWithOutputConstraint}

% Simulation results of comparing the dual-loop controller concerning output constraints with that not considering output constraints are shown in Figure \ref{fig:ConstraintComparison}. In Figure \ref{fig:2-norm_constraint_violation}, the 2-norm constraint violation for layer $k$ is defined as

% \begin{equation}
%     g_k(\rho) = \norm{\rho_{\text{up},k} + \rho_{\text{low},k}}_2
%     \label{eqn:OutputPenaltyInSimulation}
% \end{equation}
% where
% \begin{equation}
% \begin{aligned}
%     \rho_{\text{up},k} = \Bigl[&\max{\Bigl(y_k[3]-(y_d+\rho), 0\Bigl)}, ..., \\
%     &\max{\Bigl(y_k[l_p]-(y_d+\rho), 0\Bigl)}\Bigl]^T\\
%     \rho_{\text{low},k} = \Bigl[&\max{\Bigl((y_d-\rho)-y_k[3], 0\Bigl)}, ..., \\
%     &\max{\Bigl((y_d-\rho)-y_k[l_p], 0\Bigl)}\Bigl]^T\\
%     \label{eqn:OutputPenaltyTermClarificationInSimulation}
% \end{aligned}
% \end{equation}

% It can be seen that in almost all testing metrics, the dual-loop controller with output constraints surpasses the one without output constraint, which might be counter-intuitive because a trade-off between minimizing the mean absolute error and the constraint violation is expected. One possible speculation is that the introduced output penalty helps optimize control gains by finding a better gradient descent path for minimizing the mean absolute error and prevent it from falling into a local minima. Future work may focus on rigorously testing this conjecture.

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{graphics/MeanAE_constraint.pdf}
%         \caption{}
%         \label{fig:MeanAE_constraint}
%         \end{subfigure}
%     \hspace{1mm}
%     \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{graphics/MaxAE_constraint.pdf}
%         \caption{}
%         \label{fig:MaxAE_constraint}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{graphics/2-norm_constraint_violation.pdf}
%         \caption{}
%         \label{fig:2-norm_constraint_violation}
%     \end{subfigure}
%     \caption{Box plots of mean absolute error (a), maximum absolute error (b), and 2-norm constraint violation (c) given by two dual-loop controllers without measurement noise. Maximum absolute errors in layer 1 for dual-loop controllers with and without constraints are $124~\text{K}$ and $140~\text{K}$ respectively. $y_d=1500~\text{K}$.}
%     \label{fig:ConstraintComparison}
% \end{figure}

Besides control accuracy, efficiency is a crucial aspect in real-world applications. Since the in-layer linear feedback control only involves additions and multiplications, its computation time can be ignored. The layer-to-layer control loop takes up to \SI{0.02}{\second} to compute $u_N^f$ by using the Clarabel solver \cite{goulart2026clarabel}, making the scheme suitable for real-world deployment.

Overall, the simulation highlights the superiority of the dual-loop controller over in-layer and layer-to-layer approaches, with a considerable computational efficiency.

==> sections/old_sections/5_real-world_experiments.tex <==
\subsection{Experimental Results} \label{Real-worldExperiments}

% We now train the dual-loop controller in simulation and test its performance on a real SLM process. Numerical values for the real process parameters are given in \cref{Tab:ProcessParametersReal,Tab:ProcessParametersRealCalibration} in \cref{sec:ModelParametersForRealMachine}. The hardware architecture we utilized is summarized in \cref{fig:SLM_hardware_setup}.

% \begin{figure}
%      \centering
%      \footnotesize
%         \import{./graphics/svgs/}{control_slm_2.pdf_tex}
%      % \vspace{5pt}
%      \caption{The utilized hardware setup.\bk{Some suggestions/corrections for the figure: the orange boxtitle to be: "Optical path". Dichroic mirror should be "dynamic focusing unit". The beam expander should be "galvo mirrors" or "scanner". The dichroic mirror is kind of where the focus lens is. The schematic is kind of accurate enough but please refer to the BO paper for a more accurate design. The blue and orange boxes to be the same height. the arrow on the powder reserve (whic could be "powder supply as well") should point up, not down. The excess powder bit shouldnt have an arrow at all. the recoater should be a thin-ish rectangle, not a cylinder.}}
%      \label{fig:SLM_hardware_setup}
% \end{figure}

% The training of the feedback gains is done in simulation similar to what was done in Section \ref{SimulationExperiments}, but in \cref{eqn:InLayerOptimization} the objective function is changed to
% \begin{equation*}
% J_{\text{in}}(K) = \mathbb{E}_{w,\theta'} \Bigl[~\frac{1}{t_p} \bigl( \sum_{j=1}^{t_p} \norm{y_1[j] - y_d}^2 + \lambda \sum_{j=0}^{t_p-1} \bigl[u_{\text{min}}-u_1[j] \bigl]_+ + \bigl[u_1[j]-u_{\text{max}} \bigl]_+ \bigl)~\Bigl]
% \end{equation*}
% in which $\lambda$ is the input constraint violation penalty coefficient, $[x]_+ = \operatorname{max}(0,x)$, and the constraint $u_1[t] = u_1^f[t]+u_1^b[t]$ is formulated without the Euclidean projection $\Pi_{U}$, because in the real SLM process there is no hard constraint on the input. However, we expect the input to stay within $[u_\text{min}, u_\text{max}]$ as much as possible to prevent the lack of fusion (happens when the input drops below $u_\text{min}$) and keyholing (happens when it exceeds $u_\text{max}$), and therefore we add the input constraint violation penalty term in the objective function.

% In addition, limited by the capability of the machine, we make the following simplifications: (1) the layer-to-layer control loop produces a single feedforward input that remains constant throughout the entire layer, that is, $u_N^f[t]=u_N^f[0]$ for all $t=0,\dots,t_p-1$, (2) the in-layer control loop is substituted by a proportional-integral (PI) controller of the form
% \begin{equation*}
%     u_{N}^b[t]=K_{p} e_{N}[t] + K_i \Delta t \sum_{i=0}^{t} e_{N}[i].
%     %\label{eqn:PIController}
% \end{equation*}
% %
% % For real-world experiments, we aim to make use of the constructed control-oriented model and the dual-loop control scheme to realize feedback tuning in simulation environment, and then directly deploy them to real SLM machines to showcase the robustness of the proposed control scheme. However, limited by the capability of the machine, we make the following simplifications: (1) The layer-to-layer control loop is substituted by an input with nominal power, (2) The in-layer control loop is substituted by a proportional-integral (PI) controller.
% %
% The full input is therefore given by
% \begin{equation}
%     u_{N}[t] = u^f_N[0] + u_N^b[t]. \\
%     \label{eqn:FullInputReal}
% \end{equation}
% %
% With these simplifications, our controller becomes a PI controller with a feed-forward term, as previously studied in the literature \cite{shkoruta2022real,kavas2024situ}. Unlike these works, however, here the tuning is performed in simulation, eliminating the need for real experimental data and significantly reducing costs.
% %
% %These simplifications turn the controller into a PI controller with static feed-forward input, which might be treated the same as previous research such as \cite{Image-based-feedback-control, kavas2024situ}. 
% %This validates the accuracy of the constructed model, bringing insights for much cheaper feedback tuning methods.

% \begin{figure}
%      \centering
%      \includegraphics[width=.6\textwidth]{graphics/wedge_path_new.pdf}\\
%      \caption{Wedge path for the laser. The laser scans from right to left, with hatching proceeding from top to bottom.}\label{fig:WedgePath}
% \end{figure}

% \begin{figure}
%      \centering
%      \captionsetup{skip=0pt}
%      \input{graphics/tex/wedge_sim_real_regress.tex}\\
%      \caption{Linear regression between simulation output $y_\text{sim}$ and real output $y_\text{real}$, with $y_\text{sim} = 0.1469 y_\text{real} -142.2$, and $r^2=0.6371$.} \label{fig:SimRealRegression}
% \end{figure}

% % and $y_{\text{sim}}=3.032y_{\text{real}}+565.352$}

% \begin{figure}
%      \centering
%      \captionsetup{skip=0pt}
%      \input{graphics/tex/wedge_sim_real_fit.tex}\\
%      \caption{Similarity analysis between mapped simulation output and real output, in which the former one is generated by the linear regression in \cref{fig:SimRealRegression}. MSE=188.3.} \label{fig:SimRealSimilarity}
% \end{figure}

% To compare with the state-of-the-art control scheme of \cite{kavas2024situ}, we consider the ``wedge" path in \cref{fig:WedgePath}, used in \cite{kavas2024situ}, which also shows significant in-layer overheating problems. Moreover, for consistency with \cite{kavas2024situ}, the PI controller's integral term is only accumulated for vectors where the laser is on.

% \subsection{Training Setting for In-layer Control Loop in Simulation}\label{sec:TrainingSettingForInLayerControlInSimulation}

% We train the proportional gain $K_p$, integral gain $K_i$, and the feedforward term $u_N^f[0]$ by gradient descent. The batch size is 1, and for each training epoch, 1 model with uncertain parameters $e_\alpha, e_\epsilon, e_\kappa$ uniformly sampled from the interval $[-0.1, 0.1]$ is used to construct the system dynamics. The initial values of $K_p$ and $K_i$ are set a little bit larger than 0 to avoid the influence of large gradient on the momentum of the optimizer at the beginning of the training, and the initial value of $u_N^f[0]$ is $\SI{150}{W}$. We trained for 200 epochs with 1 update in each epoch, taking approximately 63 minutes in total on a NVIDIA GeForce RTX 3050 Ti GPU. The Adam optimizer is used for gradient descent \cite{kingma2014adam}.
% %, with learning rate for $K_p, K_i,$ and $u_N^f[0]$ set to $\num{2e-2}, \num{1e-3},$ and $\num{1}$ respectively, such that their training speed can be balanced even though they have different gradient scales.
% The measurement noise $w \sim \text{Uniform}[\SI{-5}{\kelvin},\SI{5}{\kelvin}]$ is drawn randomly for each time step in the printing process to improve the robustness of the in-layer controller. The desired temperature $y_d$ is set to \SI{1523.2}{\kelvin}, corresponding to \SI{80}{\milli\volt} output signal for the real process.

% % We highlight one practical consideration for the real experimental setup:
% %(1) the printing time in the real experiments ($0.12854\,\si{\second}$) is substantially longer than the simulation time in Section \ref{SimulationExperiments} ($0.00125\,\si{\second}$), yet the sampling interval remains identical. To expedite training, we therefore utilize only the final 25 scans of the wedge (out of 50), discarding the initial scans where overheating is negligible. This approach better targets the severe overheating regime.
% % For consistency with \cite{kavas2024situ}, we apply no filter during the temperature control, and therefore the Butterworth filter introduced in \cref{sec:TestingSettingForDualLoopControlScheme} is discarded. For the same consideration, the PI controller's integral term is only accumulated for scans where the laser is on.

% \subsection{Calibration}\label{sec:Calibration}

% The output of the SLM machine used in the experiments is a signal measured in millivolt (\si{\milli\volt}), as stated in \cite{kavas2024situ}. This differs from the output of the simulation, which is in Kelvin (\si{\kelvin}). To ensure that the simulation correctly describes the dynamics of the machine, we calibrate the parameters of the simulation by running a grid search for different possible parameter sets before training. For each parameter set, we use linear regression to map the simulated signals to the real signals, and calculate the mean squared error (MSE) between the mapped simulated signals and real signals. In the end, the parameter set (listed in \cref{Tab:ProcessParametersRealCalibration} in \ref{sec:ModelParametersForRealMachine}) with lowest MSE is chosen. \jl{should justify a bit why kp > kd?} This procedure only requires data collected on a single scan, with constant input power.

% The linear regression between the simulated output and the real output  is shown in Figure \ref{fig:SimRealRegression}. The similarity analysis between the mapped simulated output and the real output are shown in Figure \ref{fig:SimRealSimilarity}. \jl{Note that due to the lack of memory for storing tex files in overleaf, I only pick 1/4 data for fig 8 and 9 drawing. Need to include all data points or not?}

%Due to the difference of the input and output unit between simulation environment and real machines, parameter fitting is done as follows.
%
%In terms of input, the simulation environment uses Watt (\si{\watt}) as unit while the real machine uses digital signal, in which \num{0} corresponds to \SI{0}{\watt} and \num{4096} corresponds to \SI{500}{\watt}. A linear relationship can be easily constructed to transform the input between simulation and real world.
%
%In terms of output, the simulation environment uses Kelvin (\si{\kelvin}) as unit while the real machine uses millivolt (\si{\milli\volt}), as stated in \cite{kavas2024situ}. We apply same input to the simulation and the real machine and adjust our simulation parameters in Table \ref{Tab:ProcessParameters} such that the linear regression has a large coefficient of determination ($r^2$). The linear regression result and the corresponding similarity analysis are shown in Figure \ref{fig:SimRealRegression} and \ref{fig:SimRealSimilarity} respectively.

% \subsection{Simulation Results}\label{sec:SimulationResultsRealWorld}

% Simulation results between feed-forward 150 W input (150W) and that with a PI controller (150W+PI) can be seen in Figure \ref{fig:MeanAERealWedge} and \ref{fig:EnvelopeRealWedge}, in which the trained PI controller has $K_p=11.30, K_i=21857.56$. Although the PI controller leads to a bit larger mean absolute error for cases with small mean absolute error (i.e. cases with small model mismatch), it greatly reduces the error for cases with large mean absolute error (i.e. cases with large model mismatch). Also, Figure \ref{fig:EnvelopeRealWedge} demonstrates that the increase of mean absolute error for PI controller mainly comes from the beginning of each scan, which is expected.

% \begin{figure}
%      \centering
%      \includegraphics[width=.35\textwidth]{graphics/MeanAE_real_wedge_no_noise.pdf}\\
%      \caption{Box plot of mean absolute error given by nominal feed-forward input and that with PI controller. $y_d=750~\text{K}$ }\label{fig:MeanAERealWedge}
% \end{figure}

% \begin{figure}
%      \centering
%      \includegraphics[width=.5\textwidth]{graphics/envelope_plot_real_wedge_no_noise.pdf}\\
%      \caption{Upper and lower bounds of all tested outputs derived by feed-forward 150 W input and that with a PI controller without measurement noise. $y_d=750~\text{K}$ }\label{fig:EnvelopeRealWedge}
% \end{figure}

\subsection{Real-world test results}\label{sec:Real-worldTestResults}

After training we obtain
\begin{align*}
K_p=15.77,~~ K_i=13201.82,~~ u_N^f[0]=162.77W.
\end{align*}
In \cite{kavas2024situ}, the chosen PI parameters $K_p=8.45, K_i=90598.24$ are obtained offline for the controller (thereafter referred to as ``BayesOpt") through real-world tuning, without feedforward static input. The objective of both controllers is to drive the output signal as close to \SI{80}{\milli\volt} as possible throughout the print of each layer. 

The test results are shown in \cref{fig:RealComparison}. To improve the clarity, only the results for vectors where the laser is on are presented. The top row of subplots displays the pyrometer signal (in mV) across the printing window. The signal is first smoothed using a moving horizon filter with a window size of $100$ time steps, and then averaged across layers $50$ to $80$. Observe how both BayesOpt (left) and our method (center) effectively eliminate the severe overheating that occurs when a constant power profile is used (right).

The performance of our method closely matches that of BayesOpt, with a slight decrease in the output error ($4.63\,\text{mV}$ compared to $4.65\,\text{mV}$, as shown in the bottom row of subplots). Moreover, the power profile obtained with our method stays significanly closer to the desired operating range $140\,\text{W}$-$210\,\text{W}$ (the band between the dashed green and yellow lines in the second row of subplots), reducing the mean input violation error from $15.43\,\text{mV}$ to $6.76\,\text{mV}$. 
By keeping the input within this range, we expect our controller to better prevent both lack of fusion (when the input drops below the green line) and keyholing (when it exceeds the yellow line).
The results also suggest potential applications where a range of input values are specifically desired for another control target (i.e. solidification rate or thermal gradient objectives) while controlling the melt pool emissions.

%\jl{Delete this paragraph since we don't have 110 mV test anymore?} To further evaluate the generalizability of our method, we applied the controllers on the same experimental setup using a reference of $110\,\text{mV}$. 
The corresponding results are reported in the bottom half of \cref{fig:RealComparison}. 
% \bk{can we add any further discussion statements about the generalization capacity of the controller or the parameters? like, "tuning for a single ref value is enough" etc.?} 
%The observed outcomes are consistent with those obtained for the $80\,\text{mV}$ reference case. 
%This supports the idea, already expressed in \cref{sec:SimulationResults}, that our controller is robust to variations of the problem parameters. 
%Together with the 80mV reference value results, further research is needed to identify various different factors (i.e. reference value, part geometry, ranges of scan vector lengths, etc.) to obtain optimum controller for the LPBF process. \rz{I don't get this comment.}

\begin{figure*}
     \centering
     \captionsetup{skip=0pt}
     %
     \begin{subfigure}[c]{\textwidth}
          \centering
          \includegraphics{graphics/real_scans/scans_mean_80mV.pdf}
     \end{subfigure}\\
     % \vspace{1sp}
     % \begin{subfigure}[c]{\textwidth}
     %      \centering
     %      \includegraphics{graphics/real_scans/scans_mean_110mV.pdf}
     % \end{subfigure}
     \caption{Time series comparison of pyrometer signals across wedge specimens using offline-optimized BayesOpt (left column), our controller (center column), and the uncontrolled setup (right column) for reference value of $80\,\text{mV}$. 
     %(above) and $110\,\text{mV}$ reference (below).
     For clarity, only the results for scans where the laser is on are presented. Each curve represents the average signal over layers $50$ to $80$, smoothed using a moving average filter with a window size of $100$ time steps. Shaded regions denote the standard deviation across layers. The second row visualizes the power input profiles, where the mean violation quantifies the average extent to which laser power exceeds the keyhole onset threshold or falls below the lack of fusion threshold.}\label{fig:RealComparison}
     % \bk{fontsizes of the texts within the plots are too small, they can match the rest of the fonts in size. maybe legends as well. the middle column title is still "Ours". time axis to be ms instead of $\mu$s?}
\end{figure*}

\begin{figure*}
     \centering
     \captionsetup{skip=0pt}
     \includegraphics[width=\textwidth]{graphics/scatter_28.pdf}
     % \includegraphics[width=\textwidth]{example-image-duck}
     \caption{\jl{TODO!!!} \bk{PLACEHOLDER FOR THE SCATTER PLOT (MAY BE COMBINED WITH MICROGRAPHS)}} \label{fig:RealComparisonScatter}
\end{figure*}


\begin{figure*}
     \centering
     \captionsetup{skip=0pt}
     \includegraphics[width=\textwidth]{graphics/real_scans/printed_part_images/penalty_100/BO_vs_penalty_100.jpg}
     % \includegraphics[width=\textwidth]{example-image-duck}
     \caption{\bk{PLACEHOLDER FOR 3D images}} \label{fig:3d_images}
\end{figure*}

% \begin{figure*}
%      \centering
%      \captionsetup{skip=0pt}
%      \includegraphics[width=\textwidth]{graphics/real_scans/printed_part_images/penalty_100/penalty_100_micro.jpg}
%      % \includegraphics[width=\textwidth]{example-image-duck}
%      \caption{\bk{PLACEHOLDER FOR microstructure image}} \label{fig:3d_images}
% \end{figure*}

\begin{figure*}[t]
    \centering
    \captionsetup{skip=0pt}
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphics/real_scans/printed_part_images/penalty_100/penalty_100_micro.jpg}
        \caption{\bk{PLACEHOLDER FOR microstructure image IF NOT SHOWN TOGETHER WITH THE SCATTERS} THIS ONE IS PENALTY 100}
        \label{fig:micro_image}
    \end{minipage}%
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphics/real_scans/printed_part_images/BO/BO_micro.jpg}
        \caption{\bk{PLACEHOLDER}(THIS ONE IS BO)}
        \label{fig:second_image}
    \end{minipage}
\end{figure*}

\begin{figure*}
     \centering
     \captionsetup{skip=0pt}
     \includegraphics[width=\textwidth]{graphics/real_scans/printed_part_images/porosity.png}
     % \includegraphics[width=\textwidth]{example-image-duck}
     \caption{Porosities \bk{PLACEHOLDER FOR THE SCATTER PLOT}} \label{fig:porosity}
\end{figure*}


Comments from Baris:

\begin{itemize}
    \item vector beginning surge due to the excessive energy input is really bad in uncontrolled and BO parts.
    This is due to the unidirectional hatches due to overlapping meltpool initiation transients that accumulate across layers and result in swelling. 
    Controlled ones are better, since they regulate the input by penalizing against parameter window violation for high energy input etc.
    This effect is observed in 1) Upper surface profile with vector start region swelling, 2) vector beginnings in micrographs (the larger grain region).
    \item The first vector and it's beginning of the BO is exceptionally bad(see the micrograph and 3D isometric image), which isn't the case in the uncontrolled. Our controller solved this issue as well all altogether.
    \item the length of the vector beginning no-porosity and large-grain regions can be compared to show how our controller is doing better than uncontrolled AND BO.
    \item The tip of the uncontrolled part is not following the actual geometry (it sticks out outside, see the micrograph for the uncontrolled part) due to the vector initial transient swelling. This is solved nicely by our controller as well. This is an "the controller can print the requested geometry more conforming" argument. AM people would like it.
    \item Porosity is definitely better in the new controlled ones compared to BO, yet still worse than the uncontrolled (See micrographs). It's because we again penalize the input violation, also for the lower parameter window limit.
    (Some porosity distribution statistics can be plugged in here, like the size and count of the pores, being much better than BO)
    \item Some further discussion can be made on the globular key-hole-like gas pores and lack of fusion pores.
    \item Can we say anything meaningful about punishing the out-of-limit input compared to defining hard input limits? Leaving this here as a discussion idea, food for thought.

\end{itemize}










% The test results are illustrated in Figure \ref{fig:RealComparison}. Compared with the uncontrolled scheme, our controller achieves much smaller output error with acceptable input violation magnitude. Although the output error is slightly higher than that of  BayesOpt, our method achieves a lower input violation. This reflects a more conservative and safety-aware control behavior, which is advantageous in real-time applications where constraint adherence is critical.

% \begin{figure}
%      \centering
%      \includegraphics[width=0.45\textwidth]{graphics/real_output_comparison.pdf}
%      \vskip 5pt
%      \includegraphics[width=0.45\textwidth]{graphics/real_input_comparison.pdf}
%      \vskip -3pt
%      \caption{Comparison between the output (upper) and the input (lower) of our controller and BayesOpt. A moving average with a 100-sample window is applied to the all curves.}
%      \label{fig:RealComparison}
% \end{figure}

% - Analysis of the signals across layers. Mean and 1 sigma of the mean signals across layers
%     -this is to be visualized for layers + different references.
%     -one case could be shown as an example.
%     - machine block diagram showing PID implementation.



% - different references are hard to justify. We'll keep going with 80mV
%     - Show the difference between controllers at different references. 
% - BO vs ff to be compared, qualitatively and "maybe" quantitatively.
%     - rmse comparison BO and ff to be compared, across all layers.
% - cut up ONLY if the porosity is better in ff
% - baris to intro

% \textcolor{blue}{2 questions: 1. What kind of results can be appropriately presented? I remember Efe said "mean input constraint violation" is not a proper aspect to do comparison since BayesOpt didn't take it into account.  2. In which way should the results be presented? I refer to Fig. 11 in \cite{kavas2024situ} to draw the output-time and input-time curves for Ours and BayesOpt in \cref{fig:RealComparison}. Don't know if these two plots are meaningful enough. Should I remove the moving average effect in the plots?}

% \begin{table}[htbp]
%     \renewcommand{\arraystretch}{1.2} % Adjust row spacing
%     \caption{Real-world test results of single-layer printing}
%     \centering
%     \begin{tabularx}{\columnwidth}{|c| *{4}{>{\centering\arraybackslash}X|}}
%         \hline
%         \multirow{2}{*}{Controller} & \multicolumn{4}{c|}{Mean Absolute Error [\si{\milli\volt}]}\\ \cline{2-5}
%         & 1  & 2  & 3 & Average \\ 
%         \hline
%         Ours  & 11.2752 & 10.8260 & 10.8578 & 10.9923\\
%         \hline
%         BayesOpt  & 11.0713 & 11.0425 & 10.6074 & 10.9071 \\ 
%         \hline
%     \end{tabularx}
%     \begin{tabularx}{\columnwidth}{|c| *{4}{>{\centering\arraybackslash}X|}}
%         \hline
%         \multirow{2}{*}{Controller} & \multicolumn{4}{c|}{Mean Input Constraint Violation [\si{\watt}]}\\ \cline{2-5}
%         & 1  & 2  & 3 & Average \\ 
%         \hline
%         Ours  & 3.6454 & 3.5513 & 3.3600 & 3.5189\\
%         \hline
%         BayesOpt  & 8.8408 & 8.5419 & 7.5463 & 8.3097 \\ 
%         \hline
%     \end{tabularx}
%     \label{Tab:RealWorldTestResults}
% \end{table}

% \subsection{Real-world test results of multiple-layer printing}\label{sec:Real-worldTestResultsMultiple}

% In this subsection, we aim to test the performance of our PI controller (still with $K_p=11.30$ and $K_i=21857.56$) across multiple layers of wedge printing. The objective of the controller is to drive the output signal as close to 80 mV as possible throughout the printing of $N=33$ layers. 
% % Besides testing on the wedge path in which the scanning direction is the same throughout the printing of a single layer, as demonstrated in Figure \ref{fig:WedgePath}, we also test on the wedge path with alternating scanning directions to show the robustness of our controller. The details of the tested wedge paths can be seen in Figure \ref{fig:RealWedge}, and the test results are summarized in \cref{Tab:RealWorldTestResultsMulti}.

% The test results are summarized in \textcolor{red}{TODO}.

% \begin{figure}
%      \centering
%      \captionsetup{skip=4pt}
%      \includegraphics[width=.15\textwidth]{graphics/real_wedge.pdf}\\
%      \caption{Tested wedge paths, in which wedge 1 and 2 are with the same scanning direction throughout printing, and wedge 3 to 6 are with alternating scanning directions.} \label{fig:RealWedge}
% \end{figure}

% \begin{table}[htbp]
%     \renewcommand{\arraystretch}{1.2} % Adjust row spacing
%     \caption{Real-world test results of multi-layer printing \textcolor{red}{TODO}}
%     \centering
%     \begin{tabularx}{\columnwidth}{|c| *{4}{>{\centering\arraybackslash}X|}}
%         \hline
%         \multirow{2}{*}{Controller} & \multicolumn{4}{c|}{Mean Absolute Error [\si{\milli\volt}]}\\ \cline{2-5}
%         & 1  & 2  & 3 & Average \\ 
%         \hline
%         Ours  & 11.2752 & 10.8260 & 10.8578 & 10.9923\\
%         \hline
%         BayesOpt  & 11.0713 & 11.0425 & 10.6074 & 10.9071 \\ 
%         \hline
%     \end{tabularx}
%     \begin{tabularx}{\columnwidth}{|c| *{4}{>{\centering\arraybackslash}X|}}
%         \hline
%         \multirow{2}{*}{Controller} & \multicolumn{4}{c|}{Mean Input Constraint Violation [\si{\watt}]}\\ \cline{2-5}
%         & 1  & 2  & 3 & Average \\ 
%         \hline
%         Ours  & 3.6454 & 3.5513 & 3.3600 & 3.5189\\
%         \hline
%         BayesOpt  & 8.8408 & 8.5419 & 7.5463 & 8.3097 \\ 
%         \hline
%     \end{tabularx}
%     \label{Tab:RealWorldTestResultsMulti}
% \end{table}

